Variable-Wise Diagonal Preconditioning for Primal-Dual Splitting: Design and Applications

This paper proposes a method for designing diagonal preconditioners for a preconditioned primal-dual splitting method (P-PDS), an efficient algorithm that solves nonsmooth convex optimization problems. To speed up the convergence of P-PDS, a design method has been proposed to automatically determine appropriate preconditioners from the problem structure. However, the existing method has two limitations. One is that it directly accesses all elements of matrices representing linear operators involved in a given problem, which is inconvenient for handling linear operators implemented as procedures rather than matrices. The other is that it takes an element-wise preconditioning approach, which turns certain types of proximity operators into analytically intractable forms. To overcome these limitations, we establish an Operator norm-based design method of Variable-wise Diagonal Preconditioning (OVDP). First, OVDP constructs diagonal preconditioners using only (upper bounds) of the operator norms of linear operators, thus eliminating the need for their explicit matrix representations. Furthermore, since OVDP takes a variable-wise preconditioning approach, it keeps any proximity operator analytically computable. We also prove that our preconditioners satisfy the convergence condition of P-PDS. Finally, we demonstrate the effectiveness and usefulness of OVDP through applications to mixed noise removal of hyperspectral images, hyperspectral unmixing, and graph signal recovery.

==> fig_tex/fig_graph2_GSR_colored.tex <==

\begin{figure*}[!t]
	\begin{center}
		\begin{minipage}{0.97\hsize}
			\centerline{\includegraphics[width=\hsize]{./figure/GS_Recovery/graphs2/graph_recovery_all_graph_loglog.eps}} %画像
		\end{minipage}
	\end{center}
	%\begin{center}
	%\begin{minipage}{0.97\hsize}
	%	\centerline{\includegraphics[width=\hsize]{./figure/GS_Recovery/graphs2/graph_recovery_all_graph.eps}} %画像
	%\end{minipage}
	%\end{center}
	
	
	\vspace{-2mm}
	
	\caption{Convergence profiles in graph singal recovery. (a): Iterations/\textcolor{red}{computational} time versus RMSE. (b): Iterations/\textcolor{red}{computational} time versus \textcolor{red}{RES}. (c): Iterations/\textcolor{red}{computational} time versus PSNR.}
	\label{fig:graph_GSR}
\end{figure*}


==> fig_tex/fig_graph2_MNR_colored.tex <==

\begin{figure*}[!t]
	\begin{center}
		\begin{minipage}{0.97\hsize}
			\centerline{\includegraphics[width=\hsize]{./figure/MNR/graphs2/HSI_mixednoise_removal_all_graph_loglog.eps}} %画像
		\end{minipage}
	\end{center}
	
	\vspace{-2mm}
	
	\caption{Convergence profiles in mixed noise removal. (a): Iterations/\textcolor{red}{computational} time versus RMSE. (b): Iterations/\textcolor{red}{computational} time versus \textcolor{red}{RES}. (c): Iterations/\textcolor{red}{computational} time versus PSNR. Note that applying P-PDS with \ASEWs (\textcolor{red}{green} dotted line) to Prob.~\eqref{prob:sstv_restoration_formulation} is not practical in terms of implementation (the linear operators $\DiffvSymb$, $\DiffhSymb$, and $\DiffbSymb$ are not usually implemented as explicit matrices).}
	\label{fig:graph_MNR}
\end{figure*}


==> fig_tex/fig_graph2_Unm_colored.tex <==

\begin{figure*}[!t]
	\begin{center}
		\begin{minipage}{0.97\hsize}
			\centerline{\includegraphics[width=\hsize]{./figure/unmixing/graphs2/unmixing_all_graph_loglog.eps}} %画像
		\end{minipage}
	\end{center}
	
	\vspace{-2mm}
	
	\caption{Convergence profiles in unmixing. (a): Iterations/\textcolor{red}{computational} time versus RMSE. (b): Iterations/\textcolor{red}{computational} time versus \textcolor{red}{RES}. (c): Iterations/\textcolor{red}{computational} time versus SRE.}
	\label{fig:graph_Unm}
\end{figure*}


==> fig_tex/fig_pds_parameters.tex <==
\begin{figure}[!t]
	\begin{center}
		\centerline{\includegraphics[width=\hsize]{./figure_ng/HSI_SSTV_destriping_result_stepsize.eps}} %画像
	\end{center}
	
	\vspace{-10mm}
	
	\caption{PDSのステップサイズに対する反復数のグラフ．横軸は$\gamma_{1}$の値，縦軸は収束基準を満たすまでの反復回数．}
	\label{fig:pds_parameters}
\end{figure}

%\begin{figure}[!t]
%	\begin{center}
%		\centerline{\includegraphics[width=\hsize]{./figure/HSI_SSTV_destriping_result_stepsize.eps}} %画像
%	\end{center}
%	
%	\vspace{-10mm}
%	
%	\caption{PDSのステップサイズに対する反復数のグラフ．横軸は$\gamma_{1}$の値，縦軸は収束基準を満たすまでの反復回数．}
%	\label{fig:pds_parameters}
%\end{figure}

==> fig_tex/fig_pds_vs_ours.tex <==
%\begin{figure*}[!t]
%	\begin{center}
%		\begin{minipage}{0.32\hsize}
%			\centerline{\includegraphics[width=\hsize]{./figure_ng/HSI_SSTV_destriping_result_converge_rate.eps}} %画像
%		\end{minipage}
%		\begin{minipage}{0.01\hsize}
%			~
%		\end{minipage}
%		\begin{minipage}{0.32\hsize}
%			\centerline{\includegraphics[width=\hsize]{./figure_ng/HSI_SSTV_destriping_result_function_value.eps}} %画像
%		\end{minipage}
%	\end{center}
%	
%	\caption{PDSと我々の手法の比較．左の図が反復数に対する変数と解の距離$\sqrt{\|\bar{\mathbf{u}} - \mathbf{u}^{(n)}\|_{2}^{2} + \|\bar{\mathbf{s}} - \mathbf{s}^{(n)}\|_{2}^{2} }/(n_{1}n_{2}n_{3})$．右図が関数の値の推移．}
%	\label{fig:pds_vs_ours}
%\end{figure*}

\begin{figure*}[!t]
	\begin{center}
		\begin{minipage}{0.32\hsize}
			\centerline{\includegraphics[width=\hsize]{./figure/SSTV_destriping_result_convergence_rate_PDSs_and_Ours.eps}} %画像
		\end{minipage}
		\begin{minipage}{0.01\hsize}
			~
		\end{minipage}
		\begin{minipage}{0.32\hsize}
			\centerline{\includegraphics[width=\hsize]{./figure/SSTV_destriping_result_function_values_PDSs_and_Ours.eps}} %画像
		\end{minipage}
		\begin{minipage}{0.01\hsize}
			~
		\end{minipage}
		\begin{minipage}{0.32\hsize}			\centerline{\includegraphics[width=\hsize]{./figure/SSTV_destriping_result_PSNRs_PDSs_and_Ours.eps}} %画像
		\end{minipage}
	\end{center}


	\vspace{-5mm}

	\begin{center}
		\begin{minipage}{0.32\hsize}
			\centerline{(a)} %画像
		\end{minipage}
		\begin{minipage}{0.01\hsize}
			~
		\end{minipage}
		\begin{minipage}{0.32\hsize}
			\centerline{(b)} %画像
		\end{minipage}
		\begin{minipage}{0.01\hsize}
			~
		\end{minipage}
		\begin{minipage}{0.32\hsize}
			\centerline{(c)} %画像
		\end{minipage}
	\end{center}
	
	\vspace{-5mm}
	
	\caption{The comparison of PDS stepsizes~\eqref{eq:PDS_stepsizes}, R/C-AS-EW~\cite{DP-PDS}, and ON-VW (Ours). (a): NRMSE versus iteration. (b): RES versus iteration. (c): PSNR versus iteration. Note that applying P-PDS with R/C-AS-EW (yellow dotted line) to Prob. (15) is not practical in terms of implementation. (the linear operators $\mathfrak{D}_{v}$, $\mathfrak{D}_{h}$, and $\mathfrak{D}_{h}$ are not usually implemented as explicit matrices)}
	\label{fig:pds_vs_ours}
\end{figure*}

% caption ．左の図が反復数$n$に対するNRMSE（式~\eqref{eq:NRMSE}参照）の推移．右図が反復数$n$における変数の関数値と真の関数値の差（式~\eqref{eq:function_diff}）の推移

%\begin{figure*}[!t]
%\begin{center}
%	\begin{minipage}{0.32\hsize}
%		\centerline{\includegraphics[width=\hsize]{./figure/HSI_destriping_convergence_rate.eps}} %画像
%	\end{minipage}
%	\begin{minipage}{0.01\hsize}
%		~
%	\end{minipage}
%	\begin{minipage}{0.32\hsize}
%		\centerline{\includegraphics[width=\hsize]{./figure/HSI_destriping_function_value.eps}} %画像
%	\end{minipage}
%\end{center}
%
%\caption{capcap}
%\label{fig:pds_vs_ours}
%\end{figure*}

==> fig_tex/fig_result_image.tex <==
\begin{figure*}[!t]
	\begin{center}
		\begin{minipage}{0.19\hsize}
			\centerline{\includegraphics[width=\hsize]{./figure/original.eps}} %画像
		\end{minipage}
		\begin{minipage}{0.19\hsize}
			\centerline{\includegraphics[width=\hsize]{./figure/noised.eps}} %画像
		\end{minipage}
		\begin{minipage}{0.19\hsize}
			\centerline{\includegraphics[width=\hsize]{./figure/PDS_result.eps}} %画像
		\end{minipage}
		\begin{minipage}{0.19\hsize}
			\centerline{\includegraphics[width=\hsize]{./figure/RCASEW_result.eps}} %画像
		\end{minipage}
		\begin{minipage}{0.19\hsize}
			\centerline{\includegraphics[width=\hsize]{./figure/Ours_result.eps}} %画像
		\end{minipage}
		
		\vspace{2mm}
		
		\begin{minipage}{0.19\hsize}
			\centerline{(a)}
		\end{minipage}
		\begin{minipage}{0.19\hsize}
			\centerline{(b)}
		\end{minipage}
		\begin{minipage}{0.19\hsize}
			\centerline{(c) PSNR=$31.48$ [dB]}
		\end{minipage}
		\begin{minipage}{0.19\hsize}
			\centerline{(d) PSNR=$33.97$ [dB]}
		\end{minipage}
		\begin{minipage}{0.19\hsize}
			\centerline{(e) PSNR=$33.93$ [dB]}
		\end{minipage}
	\end{center}


	\vspace{-5mm}
	
	\caption{Denoising results. (a): Groundtruth. (b): Observed image. (c): Image estimated by PDS with adjusted stepsizes ($\gamma_{1}=0.01$). (d): Image estimated by P-PDS with R/C-AS-EW~\cite{DP-PDS}. (e): Image estimated by P-PDS with ON-VW (Ours).}
	\label{fig:result_image}
\end{figure*}

==> fig_tex/graph_GSR.tex <==

\begin{figure*}[!t]
	\begin{center}
		\begin{minipage}{0.30\hsize}
			\centerline{\includegraphics[width=\hsize]{./figure/GS_Recovery/graphs/graph_recovery_convergence_rate.eps}} %画像
		\end{minipage}
		\begin{minipage}{0.01\hsize}
			~
		\end{minipage}
		\begin{minipage}{0.30\hsize}
			\centerline{\includegraphics[width=\hsize]{./figure/GS_Recovery/graphs/graph_recovery_function_loss.eps}} %画像
		\end{minipage}
		\begin{minipage}{0.01\hsize}
			~
		\end{minipage}
		\begin{minipage}{0.30\hsize}			\centerline{\includegraphics[width=\hsize]{./figure/GS_Recovery/graphs/graph_recovery_PSNR.eps}} %画像
		\end{minipage}
	
	\vspace{0.5mm}
	
		\begin{minipage}{0.30\hsize}
			\centerline{\FontFig{(a1) Iterations vs RMSE}} %画像
		\end{minipage}
		\begin{minipage}{0.01\hsize}
			~
		\end{minipage}
		\begin{minipage}{0.30\hsize}
			\centerline{\FontFig{(b1) Iterations vs RES}} %画像
		\end{minipage}
		\begin{minipage}{0.01\hsize}
			~
		\end{minipage}
		\begin{minipage}{0.30\hsize}
			\centerline{\FontFig{(c1) Iterations vs PSNR}} %画像
		\end{minipage}
	
	\vspace{1mm}
	
		\begin{minipage}{0.30\hsize}
			\centerline{\includegraphics[width=\hsize]{./figure/GS_Recovery/graphs/graph_recovery_convergence_rate_time.eps}} %画像
		\end{minipage}
		\begin{minipage}{0.01\hsize}
			~
		\end{minipage}
		\begin{minipage}{0.30\hsize}
			\centerline{\includegraphics[width=\hsize]{./figure/GS_Recovery/graphs/graph_recovery_function_loss_time.eps}} %画像
		\end{minipage}
		\begin{minipage}{0.01\hsize}
			~
		\end{minipage}
		\begin{minipage}{0.30\hsize}			\centerline{\includegraphics[width=\hsize]{./figure/GS_Recovery/graphs/graph_recovery_PSNR_time.eps}} %画像
		\end{minipage}
	
	\vspace{0.5mm}
	
		\begin{minipage}{0.30\hsize}
			\centerline{\FontFig{(a2) Computational time vs RMSE}} %画像
		\end{minipage}
		\begin{minipage}{0.01\hsize}
			~
		\end{minipage}
		\begin{minipage}{0.30\hsize}
			\centerline{\FontFig{(b2) Computational time vs RES}} %画像
		\end{minipage}
		\begin{minipage}{0.01\hsize}
			~
		\end{minipage}
		\begin{minipage}{0.30\hsize}
			\centerline{\FontFig{(c2) Computational time vs PSNR}} %画像
		\end{minipage}
	\end{center}
	
	\vspace{-5mm}
	
	\caption{Convergence profiles in graph singal recovery. (a): Iterations/computatioal time versus RMSE. (b): Iterations/computatioal time versus RSE. (c): Iterations/computatioal time versus PSNR.}
	\label{fig:graph_GSR}
\end{figure*}


==> fig_tex/graph_MNR.tex <==

\begin{figure*}[!t]
	\begin{center}
		\begin{minipage}{0.30\hsize}
			\centerline{\includegraphics[width=\hsize]{./figure/MNR/graphs/HSI_mixednoise_removal_convergence_rate.eps}} %画像
		\end{minipage}
		\begin{minipage}{0.01\hsize}
			~
		\end{minipage}
		\begin{minipage}{0.30\hsize}
			\centerline{\includegraphics[width=\hsize]{./figure/MNR/graphs/HSI_mixednoise_removal_function_loss.eps}} %画像
		\end{minipage}
		\begin{minipage}{0.01\hsize}
			~
		\end{minipage}
		\begin{minipage}{0.30\hsize}			\centerline{\includegraphics[width=\hsize]{./figure/MNR/graphs/HSI_mixednoise_removal_PSNR.eps}} %画像
		\end{minipage}
		
		\vspace{0.5mm}
		
		\begin{minipage}{0.30\hsize}
			\centerline{\FontFig{(a1) Iterations vs RMSE}} %画像
		\end{minipage}
		\begin{minipage}{0.01\hsize}
			~
		\end{minipage}
		\begin{minipage}{0.30\hsize}
			\centerline{\FontFig{(b1) Iterations vs RES}} %画像
		\end{minipage}
		\begin{minipage}{0.01\hsize}
			~
		\end{minipage}
		\begin{minipage}{0.30\hsize}
			\centerline{\FontFig{(c1) Iterations vs PSNR}} %画像
		\end{minipage}
		
		\vspace{1mm}
		
		\begin{minipage}{0.30\hsize}
			\centerline{\includegraphics[width=\hsize]{./figure/MNR/graphs/HSI_mixednoise_removal_convergence_rate_time.eps}} %画像
		\end{minipage}
		\begin{minipage}{0.01\hsize}
			~
		\end{minipage}
		\begin{minipage}{0.30\hsize}
			\centerline{\includegraphics[width=\hsize]{./figure/MNR/graphs/HSI_mixednoise_removal_function_loss_time.eps}} %画像
		\end{minipage}
		\begin{minipage}{0.01\hsize}
			~
		\end{minipage}
		\begin{minipage}{0.30\hsize}			\centerline{\includegraphics[width=\hsize]{./figure/MNR/graphs/HSI_mixednoise_removal_PSNR_time.eps}} %画像
		\end{minipage}
		
		\vspace{0.5mm}
		
		\begin{minipage}{0.30\hsize}
			\centerline{\FontFig{(a2) Computational time vs RMSE}} %画像
		\end{minipage}
		\begin{minipage}{0.01\hsize}
			~
		\end{minipage}
		\begin{minipage}{0.30\hsize}
			\centerline{\FontFig{(b2) Computational time vs RES}} %画像
		\end{minipage}
		\begin{minipage}{0.01\hsize}
			~
		\end{minipage}
		\begin{minipage}{0.30\hsize}
			\centerline{\FontFig{(c2) Computational time vs PSNR}} %画像
		\end{minipage}
	\end{center}
	
	\vspace{-5mm}
	
	\caption{Convergence profiles in mixed noise removal. (a): Iterations/computatioal time versus RMSE. (b): Iterations/computatioal time versus RSE. (c): Iterations/computatioal time versus PSNR. Note that applying P-PDS with \ASEWs (grean dotted line) to Prob.~\eqref{prob:sstv_restoration_formulation} is not practical in terms of implementation (the linear operators $\DiffvSymb$, $\DiffhSymb$, and $\DiffbSymb$ are not usually implemented as explicit matrices).}
	\label{fig:graph_MNR}
\end{figure*}


==> fig_tex/graph_Unm.tex <==

\begin{figure*}[!t]
	\begin{center}
		\begin{minipage}{0.30\hsize}
			\centerline{\includegraphics[width=\hsize]{./figure/unmixing/graphs/unmixing_convergence_rate.eps}} %画像
		\end{minipage}
		\begin{minipage}{0.01\hsize}
			~
		\end{minipage}
		\begin{minipage}{0.30\hsize}
			\centerline{\includegraphics[width=\hsize]{./figure/unmixing/graphs/unmixing_function_loss.eps}} %画像
		\end{minipage}
		\begin{minipage}{0.01\hsize}
			~
		\end{minipage}
		\begin{minipage}{0.30\hsize}			\centerline{\includegraphics[width=\hsize]{./figure/unmixing/graphs/unmixing_PSNR.eps}} %画像
		\end{minipage}
		
		\vspace{0.5mm}
		
		\begin{minipage}{0.30\hsize}
			\centerline{\FontFig{(a1) Iterations vs RMSE}} %画像
		\end{minipage}
		\begin{minipage}{0.01\hsize}
			~
		\end{minipage}
		\begin{minipage}{0.30\hsize}
			\centerline{\FontFig{(b1) Iterations vs RES}} %画像
		\end{minipage}
		\begin{minipage}{0.01\hsize}
			~
		\end{minipage}
		\begin{minipage}{0.30\hsize}
			\centerline{\FontFig{(c1) Iterations vs SRE}} %画像
		\end{minipage}
		
		\vspace{1mm}
		
		\begin{minipage}{0.30\hsize}
			\centerline{\includegraphics[width=\hsize]{./figure/unmixing/graphs/unmixing_convergence_rate_time.eps}} %画像
		\end{minipage}
		\begin{minipage}{0.01\hsize}
			~
		\end{minipage}
		\begin{minipage}{0.30\hsize}
			\centerline{\includegraphics[width=\hsize]{./figure/unmixing/graphs/unmixing_function_loss_time.eps}} %画像
		\end{minipage}
		\begin{minipage}{0.01\hsize}
			~
		\end{minipage}
		\begin{minipage}{0.30\hsize}			\centerline{\includegraphics[width=\hsize]{./figure/unmixing/graphs/unmixing_PSNR_time.eps}} %画像
		\end{minipage}
		
		\vspace{0.5mm}
		
		\begin{minipage}{0.30\hsize}
			\centerline{\FontFig{(a2) Computational time vs RMSE}} %画像
		\end{minipage}
		\begin{minipage}{0.01\hsize}
			~
		\end{minipage}
		\begin{minipage}{0.30\hsize}
			\centerline{\FontFig{(b2) Computational time vs RES}} %画像
		\end{minipage}
		\begin{minipage}{0.01\hsize}
			~
		\end{minipage}
		\begin{minipage}{0.30\hsize}
			\centerline{\FontFig{(c2) Computational time vs SRE}} %画像
		\end{minipage}
	\end{center}
	
	\vspace{-5mm}
	
	\caption{Convergence profiles in unmixing. (a): Iterations/computatioal time versus RMSE. (b): Iterations/computatioal time versus RES. (c): Iterations/computatioal time versus SRE.}
	\label{fig:graph_Unm}
\end{figure*}


==> tab_tex_ver2/tab_convergence_conditions_ver2_colored.tex <==

\begin{table}[t]
	\begin{center}
		\caption{Stopping Criteria.}
		\label{tab:convergence_conditions}
			%\small
			%		\tiny
			\vspace{-2mm}
			\color{red}
			\begin{tabular}{cc}
				%			\footnotesize
				\toprule
				Applications & Stopping criteria \\
				\cmidrule(lr){1-1}\cmidrule(lr){2-2}
				Mixed noise removal & $\mathrm{RMSE} < 0.005$ \\
				Unmixing & $\mathrm{RMSE} < 0.01$ \\ 
				Graph signal recovery & $\mathrm{RMSE} < 0.001$ \\
				\bottomrule
			\end{tabular}
		\color{black}
	\end{center}
	\vspace{-3mm}
\end{table}



==> tab_tex_ver2/tab_iterations_and_times.tex <==
% Iteration
\begin{table}[t]
	\begin{center}
		\caption{収束条件を満たすまでの反復数と時間(s)}
		\label{tab:iterations_and_times}
		%		\begin{tabular}{|c|c|c|cc|c|c|cc|c|c|c|c|}
		\begin{tabular}{ccc}
			\toprule
			手法 & 反復数 & 時間 (s)\\
			\cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3}
			PDS ($\gamma_{1}=0.1$) & 646 & 118.3\\
			Ours & 706 & 129.7\\
			\bottomrule
		\end{tabular}
	\end{center}
\end{table}
